HOI-Swap: Swapping Objects in Videos with Hand-Object Interaction Awareness

We study the problem of precisely swapping objects in videos, with a focus on those interacted with by hands, given one user-provided reference object image. Despite the great advancements that diffusion models have made in video editing recently, these models often fall short in handling the intricacies of hand-object interactions (HOI), failing to produce realistic edits -- especially when object swapping results in object shape or functionality changes. To bridge this gap, we present HOI-Swap, a novel diffusion-based video editing framework trained in a self-supervised manner. Designed in two stages, the first stage focuses on object swapping in a single frame with HOI awareness; the model learns to adjust the interaction patterns, such as the hand grasp, based on changes in the object's properties. The second stage extends the single-frame edit across the entire sequence; we achieve controllable motion alignment with the original video by: (1) warping a new sequence from the stage-I edited frame based on sampled motion points and (2) conditioning video generation on the warped sequence. Comprehensive qualitative and quantitative evaluations demonstrate that HOI-Swap significantly outperforms existing methods, delivering high-quality video edits with realistic HOIs.

==> rebuttal.tex <==
\setcounter{page}{1}
\newpage
\renewcommand{\thetable}{R\arabic{table}}
\renewcommand{\thefigure}{R\arabic{figure}}


\begin{table}[!t]
\tablestyle{8pt}{1.15}
  \caption{Video editing results using two new splitting ways: split by subject and action.}
  \label{tab:result_newsplit}
  \centering
  \begin{tabular}{l|ccccc|ccccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{split by subject} & \multicolumn{5}{c}{split by action} \\
& \makecell[c]{subj.\\ cons.} & \makecell[c]{mot.\\ smth.} & \makecell[c]{cont.\\ agr.} & \makecell[c]{hand \\agr.} & \makecell{hand\\ fid.} & \makecell[c]{subj.\\ cons.} & \makecell[c]{mot.\\ smth.} & \makecell[c]{cont.\\ agr.} & \makecell[c]{hand \\agr.} & \makecell{hand\\ fid.} \\
\hline
Per-frame~[\textcolor{citecolor}{8}] & 85.6 & 95.2 & 73.6 & 63.3 & 62.9 & 84.5 & 94.7 & 82.8 & 57.6 & 71.0 \\
AnyV2V~[\textcolor{citecolor}{29}] & 67.2 & 95.3 & 68.2 & 27.7 & 10.0 & 69.8 & 94.7 & 74.6 & 30.6 & 19.9\\
VideoSwap~[\textcolor{citecolor}{18}] & 88.0 & 97.4 & 71.8 & 29.6 & 69.0 & 87.2 & 97.1 & 87.7 & 39.8 & 79.4 \\
\rowcolor{LighterGray} HOI-Swap (ours) & \textbf{90.0} & \textbf{98.2} & \textbf{80.4} & \textbf{84.4} & \textbf{90.3} & \textbf{89.6} & \textbf{97.8} & \textbf{93.3} & \textbf{77.4} & \textbf{94.6} \\
\hline
\end{tabular}
\end{table}

\begin{table}[!t]
\tablestyle{5pt}{1.15}
  \caption{Detailed video editing results: in-domain videos (left) and out-of-domain videos (right).}
  \label{tab:result_breakdown}
  \centering
  \begin{tabular}{l|ccccc|c|ccccc|c}
\hline
\multirow{2}{*}{Method} & \multicolumn{6}{c|}{In-domain videos} & \multicolumn{6}{c}{Out-of-domain videos} \\
& \makecell[c]{subj.\\ cons.} & \makecell[c]{mot.\\ smth.} & \makecell[c]{cont.\\ agr.} & \makecell[c]{hand \\agr.} & \makecell{hand\\ fid.} & \makecell[c]{user\\pref.} & \makecell[c]{subj.\\ cons.} & \makecell[c]{mot.\\ smth.} & \makecell[c]{cont.\\ agr.} & \makecell[c]{hand \\agr.} & \makecell{hand\\ fid.} & \makecell[c]{user\\pref.} \\
\hline
Per-frame~[\textcolor{citecolor}{8}] & 85.8 & 94.7 & 81.3 & 61.5 & 78.4 & 0.3 & 91.0 & 96.4 & 97.3 & 71.9 & 90.2 & 0.0\\
AnyV2V~[\textcolor{citecolor}{29}] & 73.1 & 95.5 & 70.9 & 33.2 & 27.0 & 1.7 & 68.8 & 95.7 & 62.7 & 25.6 & 26.9 & 0.0 \\
VideoSwap~[\textcolor{citecolor}{18}] & 90.5 & 97.5 & 82.3 & 38.9 & 74.8 & 0.4 & 94.4 & 98.1 & 99.6 & \textbf{81.5} & 97.1 & 2.5 \\
\rowcolor{LighterGray} HOI-Swap (ours) & \textbf{91.3} & \textbf{98.0} & \textbf{89.9} & \textbf{79.0} & \textbf{96.6} & \textbf{82.7} & \textbf{94.7} & \textbf{98.6} & \textbf{99.8} & 77.8 & \textbf{99.5} & \textbf{70.2}\\
\hline
\end{tabular}
\end{table}

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/onestage_ablation.pdf}
  \vspace*{-4mm}
  \caption{Qualitative and quantitative comparisons between a one-stage baseline~[\textcolor{citecolor}{2}] and our two-stage HOI-Swap. The one-stage model struggles with preserving the new object's identify and fails to generate accurate interaction patterns, yielding inferior quantitative performance.}
\end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.7\linewidth]{figures/sd_ablation.pdf}
  \caption{Comparison of two masking strategies. The stage-I model using a segmentation mask (row 2) only learns to fill the missing region without HOI awareness. In contrast, a square bounding box (row 3) also masks the hand-object interaction regions, requiring the model to reconstruct these interactions; this enables our stage-I model to effectively learn diverse HOI patterns from data.
  % Using a square bounding box masked image (row 3) instead of a segmentation mask (row 2), our stage-I model learns HOI patterns from training images and adapts to different objects during inference. In contrast, the segmentation mask approach (row 2) only learns to fill the missing region without HOI awareness.
  }
\end{figure}

\newpage

==> sections/1.intro.tex <==
\section{Introduction} \label{sec:intro}

\begin{figure}[!t]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/intro.pdf}
  \caption{We present HOISwap that seamlessly swaps the hand-interacting object in videos with a single user-specified object image. Accommodating potential changes in object shape and resulting affordances \KG{and grasps}, HOISwap produces videos that feature realistic hand-object interactions and remain aligned with the source video. \KG{For example, notice how the grasps change to realistically accommodate the different shapes of the bottle vs.~the bowl, and how the kettle is automatically reoriented from the reference image (left) to the output video (second row) to suit the hand motion in the source video (top row).}  HOISwap is also capable of single-frame edits; the last column compares its image editing capabilities \KG{for the kettle example} with Paint by Example~\cite{yang2023paint}, AnyDoor~\cite{chen2023anydoor}, and Affordance Diffusion~\cite{ye2023affordance}. \SXnote{TO-DO: add one set of video example}  \KGnote{the mug example is not great because the person looks like they are pinching the top of the handle rather than really holding it like a mug.  Also can these examples illustrate the need to adjust the object placement/pose (vs the reference image) better?}
  }
  \label{fig:intro}
\end{figure}


Consider a video depicting the process of a human hand picking up a kettle and moving it around (Figure~\ref{fig:intro} first row). What if we want to replace the hand-interacting object in this scene with another item specified by the user—perhaps a differently-shaped kettle (row 2), a bottle (row 3), or a bowl (row 4)? This capability—to swap the \SX{\emph{in-contact}} object in a video with another, while aligning with the original video's content—is crucial for enhancing various real-world applications. Such functionality can transform entertainment, allowing users to create novel video content without the need to re-record or engage in labor-intensive manual editing. 
% Additionally, it holds significant promise for enhancing data collection processes in fields like robotics~\cite{kapelyukh2023dall,yang2023learning}.
\SX{Additionally, it holds significant promise in fields with expensive data collection processes due to hardware constraints, such as robotics, where generative models have shown potential in enabling large-scale robot learning, thereby reducing the reliance on manually collected task-specific data~\cite{kapelyukh2023dall,yang2023learning}.}
\KGnote{since people may not be familiar with what's done there and why image generation could help - say another blurb in that sentence?  ``...fields like robotics, where researchers have shown that image...generation..."} \SXnote{revised}

However, hands are notoriously challenging to work with in image/video editing~\cite{ye2023affordance,zhang2024hoidiffusion}, posing significant hurdles in manual photoshopping and often producing unsatisfactory outputs when automated by generative models. The precise swapping of hand-interacting objects presents a unique challenge that existing diffusion models~\cite{ho2020denoising, rombach2022high, blattmann2023align,xing2023survey}, despite their advances in video editing, fail to address adequately. This difficulty arises from two main factors: the need for HOI-aware capabilities and the requirement for controllability and flexibility to align with the original video. 

%%%\KGnote{I think hands are notorious for being a problem in both manual photoshopping as well as generative model outputs... should intro draw ateention to this early on as a well-known fact?} \SXnote{added}

%%%\KGnote{consider adjusting writing here to state the reasons briefly in a list, and then unpack that list.} \SXnote{revised}

First, consider the challenge of \SX{HOI awareness}. Objects chosen for swapping often vary in their properties (e.g. shape) from the original, resulting in changes to interaction patterns. For example, as illustrated in Figure~\ref{fig:intro}, replacing the kettle from the original video with a bottle (row 3), or a bowl (row 4) necessitates adjustments in the hand's grasp patterns. While many generative inpainting methods~\cite{yang2023paint,song2023objectstitch,lu2023tf,chen2023anydoor,song2024imprint,gu2024swapanything} have been developed to insert reference objects into specific scene regions, they are generally limited to contexts where the objects are \emph{isolated}—not in contact with a human hand or other objects—and thus lack HOI awareness. 
% This limitation becomes evident in complex hand-object interaction (HOI) scenarios. 
As depicted in the \SXnote{update} column of Figure~\ref{fig:intro}, the two image inpainting approaches Paint by Example (PBE)~\cite{yang2023paint} and AnyDoor~\cite{chen2023anydoor}, either merely replicate the hand pose from the original image, or produce unnaturally occluded hands, resulting in suboptimal and unrealistic HOI patterns.

Second, \KG{consider} the challenge of alignment with the original video. Despite changes in object appearance or shape, it is crucial to maintain control over the generated video to ensure it aligns with the source video both spatially and temporally. (i) Spatial alignment: The reference object might appear in any arbitrary pose; for instance, in Figure~\ref{fig:intro} row 2, the kettle handle is on the left in the reference image, but for realistic interaction, the generated content needs to reposition the kettle handle to the right, where the hand is poised to grasp it. However, current approaches do not offer this level of control, as evidenced by the results from a hand insertion approach Affordance Diffusion (Afford Diff)~\cite{ye2023affordance} in Figure~\ref{fig:intro}. Despite being adept at generating a hand interacting with the given kettle, it does not ensure correct object placement to align with the hand context in the original image, lacking spatial alignment capability.  (ii) Temporal alignment: The goal is for the generated video to mirror the object motion trajectory of the original video. Current video editing techniques~\cite{esser2023structure,yang2023rerender,hu2023videocontrolnet,chen2023control,liang2023flowvid,wang2024videocomposer,zhang2024moonshot} generally rely on the assumption of shape invariance \KGnote{unclear-invariance wrt what?} to maintain this motion alignment. These methods utilize shape-related signals (e.g. depth maps, optical flows) from the source video to guide the generation process and thus falter when applied to edits involving objects of different shapes. \SXnote{TO-DO: do we need some evidence here?} \KGnote{I don't fully understand the point yet; can the case of what it means when this is working come out in one of the rows of Fig 1?}

% First, synthesizing realistic hand-object interactions (HOI) is particularly difficult. While many generative inpainting methods~\cite{yang2023paint,song2023objectstitch,lu2023tf,chen2023anydoor,song2024imprint,gu2024swapanything} have been developed to insert reference objects into specific scene regions, they are generally limited to contexts where the objects are \emph{isolated}—not in contact with a human hand or other objects, unlike the complex HOI interactions frequently found in egocentric videos~\cite{grauman2022ego4d}. Directly applying these approaches to edit \emph{active} objects often results in poor outcomes, such as missing, strangely positioned, or distorted hands. Moreover, the task of video editing introduces added complexities; it requires positioning the reference object in a way that aligns reasonably with the hand position in the source video. Current diffusion models notably lack this control capability.  
%\KGnote{shoudl an early figure visualize these challenges (these and below)?} 
\SXnote{TO-DO update Figure 1 to include baseline results}

% The second challenge lies in how to accommodate object shape changes between the source and target video. The majority of video editing approaches~\cite{esser2023structure,yang2023rerender,hu2023videocontrolnet,chen2023control,liang2023flowvid,wang2024videocomposer,zhang2024moonshot} impose strict constraints on object shape, relying on extracting shape-related signals (e.g., depth maps and optical flows) from the source video as conditions to guide the generation of the target video. This object shape invariance assumption is impractical in household scenarios \KGnote{I don't think we have to limit it to this.} where the desired objects for swapping often vary in shape from the original. More critically, the reference object may belong to a different category (Figure \ref{fig:intro} last 2 rows), which necessitates an adjustment in the HOI affordances. Merely replicating the hand pose from the source video is suboptimal, underscoring the need for an HOI affordance-aware generative model.

% two-stage, ease generation

To address these challenges, we introduce HOISwap, a novel video editing framework designed for precise object edits, producing affordance-aware and realistic HOI videos. We approach the challenge by posing it as a video inpainting task, and propose a fully self-supervised training framework due to the impracticality of collecting paired videos. Specifically, during training, we mask the object's region within a video and task the model with inpainting the same object into the masked area, aiming to reconstruct the original video sequence. During inference, the model receives a video with the original object masked, in combination with %different 
\KG{one or more} reference object images to generate new composition(s), thereby enabling the desired object swapping functionality. We leverage two large-scale video datasets rich in HOI scenarios, HOI4D~\cite{liu2022hoi4d} and EgoExo4D~\cite{grauman2023ego}, as training sources. 

%Next, 
Our innovation is to structure the editing process into two stages. In the first stage, we select \KGnote{ambiguous to say ``we select" - us? a user? automatically?} one HOI frame from the original video to swap in the new object. For this purpose, we train one image inpainting diffusion model on the aforementioned large-scale datasets, enabling the model to learn affordances from a diverse array of real-world HOI images. The second stage is designed to propagate the initial one-frame edit across the remaining frames. Given the potential for object shape changes, we propose to employ optical flow vectors sampled from object regions in the source video as motion alignment cues, which carry significantly less shape information than traditional dense optical flow maps.  \KGnote{sampled from object regions vs. dense not clear} We use these vectors to warp a new video sequence, with the stage-I edited frame serving as the anchor. This warping process is crucial for maintaining both spatial alignment (by preserving the shape changes established in the first stage) and temporal alignment (by accurately reflecting the motion dynamics of the original video). For this stage, we train a video diffusion network that takes the warped video as conditional input to guide the generation of the final video sequence. 

Overall, our proposed two-stage editing process effectively decomposes the overall complexity into two parts, simplifying the objectives for each stage. This division allows each stage to concentrate on its specific objectives more effectively: stage I for affordance awareness and establishing spatial alignment, and stage II for temporal alignment and preserving the spatial consistency established earlier. Each stage is independently trained for greater flexibility in application. Finally, we present two effective diffusion models for the object swapping task, and establish both the image and video editing benchmark for \emph{in-contact} \KGnote{this term should appear earlier} \SXnote{do we want to use one term throughout the paper, in-contact object / hand-interacting object, or used interchangeably} object swapping. Note that the stage-I model not only supports the video swapping process but also serves as a standalone image inpainting tool.  HOISwap consistently produces realistic HOI videos that surpass existing image/video editing methods in both qualitative and quantitative evaluations, including a human study. By extending the capabilities of generative models into the largely unexplored domain of HOI, we hope that HOISwap opens new avenues for research and practical applications in this innovative field.

\KGnote{overall comment: intro is quite detailed at explaining the full method; especially if you need space, can make this much simpler, even reducing the last 3 paras into 1 para. 
 It's also still hard for me to see (like in abstract) what we are drawing out as novelty/insight vs. existing---what's the top level takeaway on novelty we want the reviewer to catch?} 

% The first stage focuses on affordance-aware object swapping in one frame. This is achieved by training an image inpainting diffusion model that takes a reference object image and an HOI image as conditional inputs to generate HOI images featuring the reference object. The second stage is dedicated to propagating the initial one-frame edit throughout the remaining frames, ensuring alignment with the original video's motion patterns. For this purpose, we propose to extract sparse motion points from the source video, which, while minimally encoding object shape information, effectively convey motion dynamics (Figure~\ref{fig:intro} first row). This stage is realized through training a image-to-video diffusion model that conditions on one frame along with sparse motion point trajectories to generate the entire video sequence. For flexibility, we independently train the two stages of HOISwap, using large-scale egocentric video datasets, HOI4D~\cite{liu2022hoi4d} and EgoExo4D~\cite{grauman2023ego}. HOISwap consistently produces videos with natural HOIs and demonstrates superior performance in user studies compared with existing video editing baselines.
%\KGnote{break up this paragraph since it's long?  also it is descriptive of waht we do, but it doesn't have a strong explicit statement about technical novelty.  and/or what insight we have that the prior methods dealing with related tasks have overlooked.} \SXnote{revised}

% Note that we exclude expensive per-video training or video-decomposition processes, which limit the practicality of editing methods. Our model is trained once and applied at inference time, enhancing its practicality for various editing scenarios. no tuning parameters for each object, effortlessly general

% Our contributions are summarized as follows: (1) We present a fully self-supervised task formulation for swapping active objects in egocentric videos, by inpainting objects in masked scenes. (2) We develop a two-stage editing framework that synthesizes HOI videos from a user-specified reference object image and the original source video, effectively managing potential shape changes between the original and new objects. (3) We present two generative models trained on egocentric videos, along with an egocentric object editing benchmark, expanding the reach of current generative models into this previously underexplored domain. (4) HOISwap produces realistic HOI videos, greatly outperforming existing baselines both quantitatively and qualitatively.



==> sections/checklist.tex <==
\newpage

\section*{NeurIPS Paper Checklist}
\setlist[itemize]{}
% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: We clearly describe our main claims such as the findings, contributions, and results in the abstract and introduction. They match our idea, methodology, and experimental results presented in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe limitations of HOI-Swap in Supp. Section~\ref{supp_sec:limitation} and provide its failure cases in Supp. video.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the editing pipeline of HOI-Edit in detail in Section~\ref{sec:method}. Also, please see main paper Section~\ref{subsec:exp_setup} and Supp. Section~\ref{supp_sec:setup} for its full implementation details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please refer to our project website.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please see main paper Section~\ref{subsec:exp_setup} and Supp. Section~\ref{supp_sec:setup} for full experimental setup of HOI-Swap. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please see Table~\ref{tab:result_userstudy} for error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please see main paper Section~\ref{subsec:exp_setup} and Supp. Section~\ref{supp_sec:setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We strictly conform the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discussed the potential negative societal impact of this work when being used to create misleading content in Supp. Section~\ref{supp_sec:social_impact}. We also discussed possible solutions to mitigate the misuse.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The focus of our paper is on video editing, specifically swapping in-contact objects in video sequences. This application does not involve the generation of misleading information, nor does it use datasets or models prone to misuse (we train our models using HOI4D and EgoExo4D data).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please see main paper Section~\ref{subsec:exp_setup} and Supp. Section~\ref{supp_sec:setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
\fi
